Self-Supervised Vessel Enhancement Using Flow-Based Consistencies

Vessel segmentation is an essential task in many clinical applications. Although supervised methods have achieved state-of-art performance, acquiring expert annotation is laborious and mostly limited for two-dimensional datasets with a small sample size. On the contrary, unsupervised methods rely on handcrafted features to detect tube-like structures such as vessels. However, those methods require complex pipelines involving several hyper-parameters and design choices rendering the procedure sensitive, dataset-specific, and not generalizable. We propose a self-supervised method with a limited number of hyper-parameters that is generalizable across modalities. Our method uses tube-like structure properties, such as connectivity, profile consistency, and bifurcation, to introduce inductive bias into a learning algorithm. To model those properties, we generate a vector field that we refer to as a flow. Our experiments on various public datasets in 2D and 3D show that our method performs better than unsupervised methods while learning useful transferable features from unlabeled data. Unlike generic self-supervised methods, the learned features learn vessel-relevant features that are transferable for supervised approaches, which is essential when the number of annotated data is limited.

==> sections/abstract_v1.tex <==
Automated blood vessel segmentation is a vital problem in medical image analysis.
Although deep learning based supervised methods have achieved state-of-the-art performance in vessel segmentation, they typically require a lot of densely annotated data, which is expensive and laborious to obtain.
These methods do not leverage unlabeled data for weak or self supervision.
In our work, we propose a self-supervised task which uses key properties of tube-like structures to perform vessel enhancement.
This task can also act as an unsupervised vessel segmentation without using expert labels.
Experiments on publicly available datasets show that our method outperforms state-of-the-art unsupervised algorithms.
Our method also achieves competitive performance with supervised learning in domain shift, showing the robustness of the features learnt by our method.
Furthermore, we show that our features are more transferable than other self-supervised methods on a downstream supervised vessel segmentation task with limited data.

==> sections/abstract_v2_s.tex <==


Automated blood vessel segmentation is a vital problem in medical image analysis. 
%Classical unsupervised methods for vessel segmentation are 
Supervised methods for vessel segmentation, although highly accurate, require training datasets with expert annotations that are labor-intensive to obtain.
%%% This statement is inaccurate because in our paper, no unsupervised method learns from data except ours:
% Unsupervised methods, on the contrary, uses weak or self supervision to learn from unlabeled data, which is readily available.
Unsupervised methods, on the contrary, use inductive biases about the object of interest to predict the presence of the object.
However, features used in unsupervised learning are not directly transferable for a deep network to use.
In our work, we propose a novel self-supervised task which uses key properties of tube-like structures to perform vessel enhancement.
Specifically, we model a vessel as a continuous path in space and provide robust estimates for radius and direction of flow associated with each vessel point.
We explicitly handle bifurcation to ensure vessel continuity at the branching points and to prevent removal of small vessel branches as noise.
The learned representations are then used in the subsequent task of unsupervised vessel segmentation.
Experiments on publicly available 2D and 3D datasets show that our method outperforms state-of-the-art unsupervised methods and is comparable to the supervised baseline.
Furthermore, we also find gains when transferring the learned representations, by our method, from an unlabeled dataset to a downstream vessel segmentation task with limited annotated data. 






 


==> sections/conclusion_v1.tex <==
\section{Discussion and Conclusion}
% The results of Table \ref{tab:unsupervised2d} show that our method learns a better representation of vessel en
%A comparison with popular unsupervised methods (Table \ref{tab:unsupervised2d}, Fig. \ref{fig:drive}) shows that our method outputs a vesselness score that performs better on a number of metrics, with a notable increase in the Dice score.

A comparison with unsupervised methods shows that our method performs objectively better on a variety of metrics, and is robust to a minor domain shift within the imaging modality, unlike supervised methods (Table \ref{tab:unsupervised2d}).
Our method also produces very few false positives and false negatives compared to unsupervised methods like Frangi (Fig. \ref{fig:drive}).
% However, our method struggles to find tiny vessels due to a lack of contrast between the tiny vessel and its surroundings.
Since our loss functions encourage the network to learn a \textit{consistent} per-pixel output of vessel statistics like radius, orientation, and bifurcations, the network learns features that are relevant to vessels.
These features are easily transferable to a supervised vessel segmentation \textit{finetuning} task compared to state-of-the-art self-supervised tasks which learn abstract features that may or may not be useful for vessel segmentation (Fig. \ref{fig:selfsupervised}).
The bifurcation loss in our method leads to better segmentation performance in regions around bifurcations (Fig \ref{fig:3}.a), which most unsupervised vessel enhancement methods do not account for.
Our method is also robust to noise in the input (Fig \ref{fig:3}.b). \\
% This is shown in Fig. \ref{fig:selfsupervised}.
% Unlike our method, other self-supervised tasks learn abstract features that may or may not be useful for vessel segmentation.
% Due to the regularizers in the loss function, our method is resilient to increasing noise in the data.
% Moreover, the bifurcation loss leads to a better segmentation around the BP.



We proposed a self-supervised task formulation for vessel enhancement without ground truth data.
Our method uses key properties of tube-like structures such as connectivity, profile consistency, and bifurcations, to introduce inductive bias into deep learning in the form of a self-supervised learning framework.
% The formulation of our method allows flexibility in prediction of the scale and orientation of vessels.
Our framework is agnostic to imaging modality, and is robust to slight domain shift.
We showed that our method outperformed several unsupervised methods, and achieved competitive performance with supervised baselines.
We showed that our method also acts as a relevant self-supervised task for a downstream vessel segmentation task.
We experimented on well-known, publicly available datasets like DRIVE, STARE, VascuSynth and COPDGene datasets and results show the versatility of our method across all these datasets.

==> sections/contributions_v1.tex <==
%!TEX root = ../draft_v1.tex
% Contributions of the paper (last paragraph of paper)
In this work, we proposed a specifically designed self-supervised task that learns feature representation for tube-like structures at multiple scales and orientations, using large-scale unlabeled datasets. 
Unlike other unsupervised methods using fixed handcrafted features [], our method adapts the features as the dataset changes.
These features can also be transferred to a supervised learning algorithm with limited data.

We evaluate the performance of our method on real 2D datasets, and a simulated 3D dataset.
Furthermore, we provide qualitative comparison on a large-scale COPD lung CT dataset.
We also show the effectiveness of our method as a self-supervised task, by comparing the training performance with state-of-the-art self-supervised algorithms. 


==> sections/experiments_v1.tex <==
%!TEX root = ../draft_v1.tex

\section{Experiments}
To evaluate the performance of our method, we run comprehensive experiments in both unsupervised and self-supervised scenarios.
In the unsupervised scenario, we compare our method with both unsupervised and supervised baselines.
To demonstrate the robustness of our proposed self-supervised task formulation, we compare the performance of our method with a supervised baseline on a domain shift problem.
In the self-supervised setting, we compare the learnt feature representations of various self-supervised tasks by comparing the training dynamics of a downstream segmentation task.
Finally, we perform an ablation study of the bifurcation term in our self-supervised loss functions.
 %Finally, we perform a qualitative analysis of our method on 3D volumes from the COPDGene dataset.

\subsection{Datasets}
In our study, we perform experiments on both 2D and 3D datasets.
The experiments on 2D data are conducted on 2 publicly available datasets: DRIVE and STARE. 
The experiments on 3D data are conducted on the VascuSynth dataset (\citet{vascusynth}).

\textbf{DRIVE}: 
The DRIVE dataset consists of 40 retinal fundus images, divided into a training and testing set of 20 images each.
% The FOV of each image is circular with a diameter of approximately 540 pixels.
% For each image, a mask image is provided that delineates the FOV.
For the training images, a single manual segmentation of the blood vessel tree structure is available.
For the test images, two manual segmentation images of the blood vessel tree are available for each image.
For evaluation, we use only the first manual segmentation as gold standard.

\textbf{STARE}:
The STARE dataset consists of 20 retinal fundus images, each with two manually annotated blood vessel tree segmentation images.
% The slides were captured by a TopCon TRV-50 fundus camera at 35 field of view.
% Each slide was digitized to produce a 605x700 RGB image.
We use this dataset in the domain shift experiment, and as a downstream task in the self-supervised learning experiment.

\textbf{VascuSynth dataset}:
The VascuSynth dataset is a 3D dataset containing synthetically generated vascular trees.
The dataset is divided into ten groups, with each group containing 12 randomly generated images with increasing amount of bifurcations.
%The vascular tree is generated iteratively using a user-defined oxygen demand map.
In our experiments, we use Groups 1-6 for training, Group 7 for validation, and Group 8-10 for testing.
%% Describe why this is important? 
% Vessel tree segmentation is an important problem in retinal fundus images because retinal vessel segmentation can be used in the evaluation of various cardiovascular and ophthalmologic diseases such as diabetes, hypertension, arteriosclerosis and chorodial neovascularization. 

\subsection{Unsupervised learning}
For unsupervised vessel enhancement and segmentation in 2D, we use the DRIVE dataset.
For our method, we divide the set of 20 images into 16 images for training and 4 for validation.
For Frangi, we use a standard implementation in Python.
We also compare our method with a supervised learning method as an upper bound of vessel segmentation performance.
For all unsupervised methods, we determine the threshold for segmentation by choosing the value which maximizes the overall Dice score over the training set.
We compare the Area under the ROC curve (AUC), Accuracy, Dice score, Sensitivity, and Specificity.
The results are summarized in Table \ref{tab:unsupervised2d}.

\begin{table*}[htpb]
    \centering
    \renewcommand{\arraystretch}{1.3}
    \begin{tabularx}{\textwidth}{XYYYY}  \toprule
         \textbf{Method} & \textbf{AUC} & \textbf{Accuracy} & \textbf{Dice score} & \textbf{Sensitivity} \\ \hline
         Frangi \cite{frangi} & 0.93431 &	0.94269 &	0.66759 &	0.65628	\\ 
         Ours  & 0.95883 & 0.95689 & 0.74586 & 0.72178 \\  \hline
         Retina-UNet & 0.97910 &	0.95501	& 0.80904 & 0.760164 	\\
         \bottomrule
    \end{tabularx}
    \vspace{3pt}
    \caption{Evaluation of vessel segmentation on DRIVE dataset.}
    \label{tab:unsupervised2d}
\end{table*}

We also compare our method with the Frangi method on the VascuSynth dataset.
Since the synthetic data is easy to predict, we compare the methods with Gaussian noise added to the input.
We vary the level of Gaussian noise from $\sigma = 0$ to $\sigma = 0.4$ in steps of $0.1$.
The results are shown in Table \ref{tab:vascu}.
\begin{table*}[htpb]
    \centering 
    \renewcommand{\arraystretch}{1.3}
    \begin{tabularx}{\textwidth}{@{}XYYYYYYYYYY@{}} \toprule
    &
    \multicolumn{2}{c}{\textbf{AUC}} & 
    \multicolumn{2}{c}{\textbf{Accuracy}} & 
    \multicolumn{2}{c}{\textbf{Dice}} & 
    \multicolumn{2}{c}{\textbf{Sensitivity}} \\
    & \textbf{Frangi} & \textbf{Ours} 
    & \textbf{Frangi} & \textbf{Ours}
    & \textbf{Frangi} & \textbf{Ours} 
    & \textbf{Frangi} & \textbf{Ours} \\
    \hline
    $\sigma = 0$ & 0.99428 & 0.99927
    & 0.99756 & 0.99817
    & 0.79282 & 0.85285
    & 0.72658 & 0.82419 \\
    $\sigma = 0.1$ &  0.99165 & 0.99951 
    &  0.99754 & 0.99834
    & 0.79148 & 0.87409
    & 0.72587 & 0.88737 \\
    $\sigma = 0.2$ & 0.98632 & 0.99891 
    & 0.99753 & 0.99873 
    & 0.78971 & 0.89239 
    & 0.72223 & 0.89169 \\
    $\sigma = 0.3$ 
    & 0.97854 & 0.99558
    & 0.99725 & 0.99849
    & 0.75601 & 0.87203
    & 0.67648 & 0.83743 \\
    $\sigma = 0.4$ 
    & 0.95994 & 0.98395
    & 0.99625 & 0.99723
    & 0.64297 & 0.74280
    & 0.55061 & 0.66309 \\
    \bottomrule
    \end{tabularx}
    \vspace{3pt}
    \caption{Results for VascuSynth dataset with increasing levels of noise added to the input}
    \label{tab:vascu}
\end{table*}

% \begin{figure}[htpb]
%     \centering
%     \includegraphics[width=0.3\textwidth]{images/vascusynth/AUC.png}
%     \includegraphics[width=0.3\textwidth]{images/vascusynth/Accuracy.png}
%     \includegraphics[width=0.3\textwidth]{images/vascusynth/Dice.png}
%     \includegraphics[width=0.3\textwidth]{images/vascusynth/Sensitivity.png}
%     \includegraphics[width=0.3\textwidth]{images/vascusynth/Specificity.png}
%     \caption{Results for VascuSynth dataset}
%     \label{fig:vascu}
% \end{figure}

% \subsection{Domain shift}
% Without explicit supervision, our method does not perform as well as a supervised method baseline.
% However, traditional supervised learning is very sensitive to domain shift.
% Since our method makes use of general properties of the vessel structure, we hypothesize that our method is more robust to domain shift.
% To test this, we train our method and Retina-UNet on the DRIVE training dataset.
% Note that our method does not have access to ground truth labels.
% We test the performance of the networks on the STARE dataset, which is similar to the DRIVE dataset, but the image capture device and FOV regions are different.
% The methods are compared in \ref{tab:domainshift}.

% \begin{table*}[htpb]
%     \centering
%     \renewcommand{\arraystretch}{1.3}
%     \begin{tabularx}{0.8\textwidth}{XYYYY} \toprule
%         \textbf{Method} & \textbf{AUC} & \textbf{Accuracy} & \textbf{Dice} & \textbf{Sensitivity} \\ \hline
%          Frangi & 0.93031 &	0.91163 &	0.59182 &	0.70269 \\
%          Retina-UNet & 0.95411 &	0.94625 &	\textbf{0.72646} &	0.69277 \\
%          Ours & \textbf{0.95992} &	\textbf{0.95286} &	0.67801 &	\textbf{0.71728} \\
%          \bottomrule
%     \end{tabularx}
%     \caption{Performance of methods trained on DRIVE dataset and tested on STARE. Note that Frangi consistently underperforms, while our method achieves competitive results with a supervised baseline without using ground truth data.}
%     \label{tab:domainshift}
% \end{table*}

% Although the supervised baseline performs well on the test images of the DRIVE dataset, as shown in Figure \ref{tab:unsupervised2d}, the performance deteriorates in the presence of a minor domain shift.
% Our method, however, retains performance across datasets due to its generalized vessel detection framework.

\subsection{Bifurcation detection}
To compare the effect of adding two bifurcation flow fields, and a bifurcation loss to align them, we compare two variants of our method on the DRIVE dataset.
In the first variant, the training loss does not include $\mathcal{L}_b(\vb_1, \vb_2, r; I, T)$ and the vesselness doesn't include the similarity of the bifurcation flow.
For the second variant, the training loss includes both the bifurcation loss and the vesselness includes the similarity of the bifurcation flow.
Since bifurcations occur in a very small region of the image space, we propose a new metric for comparing the detection of bifurcations.
The metric simply takes bounding boxes around bifurcations, and computes the dice score within the bounding box.
We manually annotate different bounding boxes containing bifurcations, and compare the performance.
Results are shown in Table \ref{tab:bifurc}.

\begin{table*}[htpb]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabularx}{0.9\textwidth}{XY}  \toprule
    \textbf{Method} & \textbf{Dice score inside bounding boxes} \\ \hline
        Frangi & 0.52509 \\ 
        Ours (without bifurcation loss) & 0.58426 \\ 
        Ours (with bifurcation loss) & \textbf{0.62343} \\ \bottomrule
    \end{tabularx}
    \vspace{3pt}
    \caption{Comparison of methods with and without bifurcation loss terms}
    \label{tab:bifurc}
\end{table*}

\subsection{Our framework as a self-supervised task}
In this section, we compare the effectiveness of our method as a self-supervised task.
Commonly used self-supervised tasks like Context Encoder, Denoising, and Colorization do not learn the features required for vessel segmentation.
Therefore, we compare our method with other self-supervised tasks by first training networks with different self-supervised tasks on the DRIVE dataset.
Then, we perform supervised vessel segmentation on the STARE dataset as the downstream task.
To test the transferability of features, we consider a \textit{limited-data} scenario where only 4 images are provided during training, and a \textit{high-data} scenario where 16 images are provided during training.
The training dynamics of the downstream task in both scenarios is shown in Figure \ref{fig:selfsupervised}.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{images/selfsupervised/highdata.png}
    \includegraphics[width=0.48\textwidth]{images/selfsupervised/lowdata.png}
    \caption{Validation curves on supervised vessel segmentation on STARE dataset with high data scenario (left) and limited data scenario (right). In both scenarios, our method achieves the best validation dice score much faster than the other self-supervision tasks.}
    \label{fig:selfsupervised}
\end{figure}


% \subsection{Comparison with unsupervised methods}
% \subsubsection{DRIVE dataset}
% \begin{enumerate}
% \item We compare our method with other unsupervised vessel enhancement methods on the DRIVE dataset.
% \item Consists of 20 retinopathy images for training, and 20 for testing.
% \item To compute other metrics, use 5 ground truth images to find optimal threshold for all methods.
% \item Results are in Table 1.
% \item Our method produces better quality vessels and has lesser noise compared to Frangi because the other loss terms prevent over-fitting to local noise or artifacts.
% \end{enumerate}

% \subsubsection{VascuSynth dataset}
% \begin{enumerate}
% \item VascuSynth is a software for simulating volumetric images of vascular trees and generating the corresponding ground truth segmentations, bifurcation locations, branch properties, and tree hierarchy.
% \item They also provide a dataset for 10 groups, containing 12 volumes each.
% \item We use 6 groups for training, 1 for validation and 3 for testing. To check the robustness of our method, we augment the volumes with Gaussian noise with increasing values of $\sigma.$
% \item Results are in Table 4.
% \item Note that our method is more robust as the noise increases.  Adding a bifurcation term improves the metrics slightly, and there is a remarkable increase in dice scores and sensitivity.
% \end{enumerate}


% \subsection{Robust domain transfer}
% \begin{enumerate}
% \item Although our method cannot perform better than supervised methods out-of-the-box, we show that our method is more robust to domain shift.
% \item We train a supervised UNet on the DRIVE dataset. The performance on the DRIVE test set is more than any unsupervised method.
% \item However, testing the network on images from the STARE dataset shows that our method performs slightly better than supervised methods.
% \item We believe that this is because small errors in predicted radius and direction of the vessels do not lead to drastic change in vesselness scores.
% \end{enumerate}

% \subsection{Comparison with other self-supervised methods}
% \begin{enumerate}
%     \item To measure the effectiveness of our method as a self-supervised task, we train our method on the DRIVE dataset, and finetune with the STARE dataset.
%     \item We compare our method with two other self-supervised tasks, namely, context encoding, and denoising.
%     \item Training curves indicate that our method learns better feature representation that helps it converge faster in the downstream task.
% \end{enumerate}

% \subsection{Effect of test-time tracking score}
% \begin{enumerate}
% \item We also test the effect of augmenting the vesselness scores with the tracking based score described in Section ???.
% \item Results are in Table 2.
% \item It is easy to see that there are slight improvements in all metrics. The improvements are not that significant because the loss terms already handle the case of overfitting.
% \item Note that for each configuration of parameters, the metrics with and without test time tracking score augmentation are with the same network parameters.
% \end{enumerate}

% \subsection{Effect of bifurcation-based loss}
% \begin{enumerate}
% \item Normal metrics would not be able to show the improvement due to the bifurcation term because of the extreme sparsity of bifurcations (vessels are sparse in the image and bifurcations are sparse within vessels).
% \item We manually annotate bounding boxes centered around bifurcations in ground truth segmentation.
% \item For all methods, we compare the dice loss of the segmentation only in these bounding boxes.
% \item Results for all methods are shown in Table 3.
% \item We show that a lot of improvement comes from using the robust vessel metric. Moreover, the bifurcation-based vesselness metric shows an overall improvement in the dice score for bifurcations.
% \end{enumerate}


% \subsection{Ablation study of different loss functions}
% \begin{enumerate}
% \item Here we study the effect of setting different values of $\lambda_f, \lambda_i, \lambda_v$.
% \item Results are in Table 1.
% \item Using the voting based metric leads to more robust vesselness maps as compared to the cross-correlation based loss.
% \item Doesn't detect ridges and can thus detect low contrast vessels better.
% \item Qualitative results are in Figure ???.
% \end{enumerate}


==> sections/experiments_v1_s.tex <==
%!TEX root = ../draft_v1.tex

\section{Experiments}
We perform four experiments to evaluate our proposed model.
All the experiments demonstrate performance on the downstream task of vessel segmentation.
First, we compare our model against established unsupervised vessel enhancement methods, namely, Frangi~\cite{frangi}, Sato~\cite{sato}, Hybrid Hessian~\cite{hessian} and Meijering~\cite{meijering} filters on two real 2D datasets.
We also examined the performances with respect to noise sensitivity on a synthetic 3D dataset.
Second, we demonstrate the importance of the bifurcation loss, by evaluating our model in terms of a novel metric that considers a bounding box around the BP to compute the dice score.
% Third, we compare against different self-supervised learning techniques, namely, training a context encoder (\cite{}), using a pretext task of image denoising [] and colorization [].
Third, we compare against different self-supervised learning techniques, namely, context encoder~\cite{pathakCVPR16context}, denoising~\cite{vincent2008extracting}, colorization~\cite{richardECCV2016} and Models Genesis ~\cite{zhou2019models}.
% We compared our model with three common self-supervision tasks, namely, context-encoder (\citet{pathakCVPR16context}), image-denoising (\citet{vincent2008extracting}), and image-colorization (\citet{richardECCV2016}).
We evaluated the transferability of representations learned by these techniques, on a subsequent downstream supervised task.
Finally, we present a qualitative assessment of our model on a real 3D dataset. 


\textbf{Datasets:} Our experiments are conducted on publicly available 2-D retinal fundus images obtained from the DRIVE~\cite{niemeijer2004comparative} and STARE~\cite{stare} datasets. The DRIVE dataset consists of 40 images, divided into a training and testing set of 20 images each. 
%Each image is 565 by 584 pixels. 
All the images have a corresponding binary mask which delineates the circular field of view (FOV) in the image.
The testing set provides two sets of manually segmented vasculatures.
The STARE database consists of 20 images. %, each of size 700 by 605 pixels.
Each image has two sets of segmented images. 
% Both in STARE and DRIVE testing set, we used the first segmentation as the ground truth.
In both the datasets, we use the first segmentation as the ground truth.
We use the VascuSynth dataset~\cite{vascusynth} for 3D analysis.
It consists of simulated volumetric images of vascular trees with corresponding ground-truth segmentations.
The dataset is divided into ten groups, with each group containing 12 randomly generated vascular trees with increasing bifurcations.
We used first six groups for training, seventh for validation, and the rest for testing.
%% Describe why this is important? 
% Vessel tree segmentation is an important problem in retinal fundus images because retinal vessel segmentation can be used in the evaluation of various cardiovascular and ophthalmologic diseases such as diabetes, hypertension, arteriosclerosis and chorodial neovascularization. 

\subsection{Unsupervised learning}

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\textwidth]{images/drive/Figure2.pdf}
    \caption{Results on DRIVE dataset. False positives are in red, and false negatives are in green. Note that Frangi has lot more false positives because of ridge detection.}
    \label{fig:drive}
\end{figure}


In this section, we compare our model against popular vessel enhancement methods. 
All the methods take raw images as input, to produce a vessel-enhanced image as output.
The vessel-enhanced image is then segmented into a binary map, by choosing a hard threshold such that the method achieves a maximum dice score over the training dataset.
We quantitatively evaluate the segmentation result as a binary classification problem. % to identify vessel versus non-vessel pixels.
We report results on five measures, namely, area under curve (AUC) of ROC curves, accuracy (acc), dice score, sensitivity (sens) and local-accuracy (acc$^*$) as defined in~\cite{localacc}.
% For local accuracy, we dilated the ground truth mask and considered  vessel pixels as positive and regions around the vessels as negative for computing accuracy.
For local accuracy, the ground truth mask is dilated considering the vessel pixels %as positive, 
and only the regions within the dilated mask are considered for the local accuracy.

Our model is trained on the training set from DRIVE dataset.
The trained model is applied on the testing set from DRIVE dataset and the entire STARE dataset.
Table~\ref{tab:unsupervised2d} presents our comparison with popular unsupervised methods including Frangi, Sato, Hessian and Meijering filters.
Without using any annotation, our model outperforms these methods and achieves a comparable performance to Retina-UNet \cite{retinaunet}, which is a supervised learning method.% based on the U-Net architecture.
Our method also performs consistently across datasets, while the performance of Retina-UNet deteriorates on STARE dataset, in the presence of a minor domain shift.

Next, we demonstrate the robustness of our model with respect to different noise levels.
To create a test set, we corrupted the original images from VascuSynth dataset by adding a zero-mean Gaussian noise, with standard deviation  ranging from $\sigma = 0$ to $\sigma = 0.4$.
Table~\ref{tab:vascu} shows our results.
Although both methods degrade in performance with increasing noise, our method consistently outperforms the Frangi filter at all the noise levels.


\begin{table*}[htpb]
    \centering
    \renewcommand{\arraystretch}{1.3}
    \begin{tabularx}{\textwidth}{@{}XYYYYY|YYYYYYY@{}} \toprule
         \textbf{Method} 
         &
         \multicolumn{5}{c}{\textbf{DRIVE}} & 
         \multicolumn{5}{c}{\textbf{STARE}} \\ 
         & \textbf{AUC} & \textbf{Acc} &  \textbf{Acc$^*$} & \textbf{Sens} & \textbf{Dice} & \textbf{AUC} & \textbf{Acc} & \textbf{Acc$^*$} & \textbf{Sens} & \textbf{Dice}\\ \hline
         Frangi & 0.93 &	94.27 &	72.02  &	0.66 & 0.67	& 0.93  &	91.16 &	67.12  &	0.70 & 0.59 \\ 
         Sato & 0.94 & 93.67 & 71.90  & 0.70 & 0.66 & 0.94 & 91.03 & 66.52 &  0.78 &  0.58 \\
         Hessian & 0.55 & 52.90 & 60.31 & \textbf{0.89} & 0.25 & 0.53 & 46.84 & 59.24 & \textbf{0.92} & 0.21  \\
         Meijering & 0.94 & 93.83 & 72.70  & 0.72 & 0.67 & 0.94 & 90.29 & 68.11  & 0.84 & 0.58 \\
         Ours  & \textbf{0.96} & \textbf{95.69} & \textbf{75.83 }  & 0.72& \textbf{0.74} &\textbf{0.96} &	\textbf{95.29} &	\textbf{69.44} &	0.80 & \textbf{0.68}\\  \hline
         Retina-UNet & 0.98 &	95.50	&80.65  & 0.76 & 0.81  & 0.95 &	94.62 &	70.05 &	0.69 & 0.73 	\\
         \bottomrule
    \end{tabularx}
    \vspace{3pt}
    \caption{Evaluation of unsupervised vessel segmentation on DRIVE and transfer-learning on STARE dataset. Acc is the global accuracy over the entire image, Acc$^*$ is the local accuracy around the dilated vessel regions.}
    \label{tab:unsupervised2d}
\end{table*}
\begin{table*}[htpb]
    \centering 
    \renewcommand{\arraystretch}{1.3}
    \begin{tabularx}{\textwidth}{@{}XYYYYYYYYYY@{}} \toprule
    &
    \multicolumn{2}{c}{\textbf{AUC}} & 
    \multicolumn{2}{c}{\textbf{Accuracy}} & 
    \multicolumn{2}{c}{\textbf{Dice}} & 
    \multicolumn{2}{c}{\textbf{Sensitivity}} \\
    & \textbf{Frangi} & \textbf{Ours} 
    & \textbf{Frangi} & \textbf{Ours}
    & \textbf{Frangi} & \textbf{Ours} 
    & \textbf{Frangi} & \textbf{Ours} \\
    \hline
    $\sigma = 0$ & 0.99 & 1.00
    & 99.76 & 99.82
    & 0.79 & 0.85
    & 0.72 & 0.82 \\
    $\sigma = 0.1$ &  0.99 & 1.00
    &  99.75 & 99.83
    & 0.79 & 0.87
    & 0.73 & 0.89 \\
    $\sigma = 0.2$ & 0.98 & 1.00
    & 99.75 & 99.87 
    & 0.79 & 0.89 
    & 0.72 & 0.89 \\
    $\sigma = 0.3$ 
    & 0.98 & 1.00
    & 99.73 & 99.85
    & 0.76 & 0.87
    & 0.68 & 0.84 \\
    $\sigma = 0.4$ 
    & 0.96 & 0.98
    & 99.63 & 99.72
    & 0.64 & 0.74
    & 0.55 & 0.66 \\
    \bottomrule
    \end{tabularx}
    \vspace{3pt}
    \caption{Results for VascuSynth dataset with increasing levels of noise added to the input}
    \label{tab:vascu}
\end{table*}

% \begin{figure}[htpb]
%     \centering
%     \includegraphics[width=0.3\textwidth]{images/vascusynth/AUC.png}
%     \includegraphics[width=0.3\textwidth]{images/vascusynth/Accuracy.png}
%     \includegraphics[width=0.3\textwidth]{images/vascusynth/Dice.png}
%     \includegraphics[width=0.3\textwidth]{images/vascusynth/Sensitivity.png}
%     \includegraphics[width=0.3\textwidth]{images/vascusynth/Specificity.png}
%     \caption{Results for VascuSynth dataset}
%     \label{fig:vascu}
% \end{figure}

% \subsection{Domain shift}
% Without explicit supervision, our method does not perform as well as a supervised method baseline.
% However, traditional supervised learning is very sensitive to domain shift.
% Since our method makes use of general properties of the vessel structure, we hypothesize that our method is more robust to domain shift.
% To test this, we train our method and Retina-UNet on the DRIVE training dataset.
% Note that our method does not have access to ground truth labels.
% We test the performance of the networks on the STARE dataset, which is similar to the DRIVE dataset, but the image capture device and FOV regions are different.
% The methods are compared in \ref{tab:domainshift}.

% \begin{table*}[htpb]
%     \centering
%     \renewcommand{\arraystretch}{1.3}
%     \begin{tabularx}{0.8\textwidth}{XYYYY} \toprule
%         \textbf{Method} & \textbf{AUC} & \textbf{Accuracy} & \textbf{Dice} & \textbf{Sensitivity} \\ \hline
%          Frangi & 0.93031 &	0.91163 &	0.59182 &	0.70269 \\
%          Retina-UNet & 0.95411 &	0.94625 &	\textbf{0.72646} &	0.69277 \\
%          Ours & \textbf{0.95992} &	\textbf{0.95286} &	0.67801 &	\textbf{0.71728} \\
%          \bottomrule
%     \end{tabularx}
%     \caption{Performance of methods trained on DRIVE dataset and tested on STARE. Note that Frangi consistently underperforms, while our method achieves competitive results with a supervised baseline without using ground truth data.}
%     \label{tab:domainshift}
% \end{table*}
% Although the supervised baseline performs well on the test images of the DRIVE dataset, as shown in Figure \ref{tab:unsupervised2d}, the performance deteriorates in the presence of a minor domain shift.
% Our method, however, retains performance across datasets due to its generalized vessel detection framework.

\subsection{Bifurcation detection}
Vessel enhancement at bifurcation points (BP) encourages vessel continuity.
In this experiment, we demonstrate the importance of our predicted bifurcation flow fields ($\vb_1, \vb_2$) in preserving such details.
To  quantitatively measure the segmentation around the bifurcation regions, we manually annotated bounding boxes (BBs) at multiple such regions in all the images from the testing set of DRIVE dataset.
BBs are of varying sizes and are placed such that the BP is at the center of the box.
We performed an ablation study, where we didn't consider bifurcation loss in our final formulation.
Table~\ref{tab:bifurc} reports the derived dice score calculated within the extracted BBs.
Our proposed bifurcation loss significantly improved the segmentation results at the BP.

\begin{table*}[htpb]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabularx}{0.9\textwidth}{XY}  \toprule
    \textbf{Method} & \textbf{Dice score inside bounding boxes} \\ \hline
        Frangi & 0.52 \\ 
        Sato & 0.52\\
        Meijering & 0.56 \\
        Hessian & 0.24 \\
        Ours (without bifurcation loss) & 0.58 \\ 
        Ours (with bifurcation loss) & \textbf{0.62} \\ \bottomrule
    \end{tabularx}
    \vspace{3pt}
    \caption{Comparison of our method with and without the bifurcation loss.}
    \label{tab:bifurc}
\end{table*}


\subsection{Our framework as a self-supervised pretext task}
In this section, we compare the transferability of the learned representation from different self-supervised tasks onto a downstream supervised vessel segmentation task.
We compared our model with four common self-supervision tasks, namely, context-encoder~\cite{pathakCVPR16context}, image-denoising~\cite{vincent2008extracting}, image-colorization~\cite{richardECCV2016} and Models Genesis~\cite{zhou2019models}.
In \textbf{context-encoder} the network learns to inpaint missing parts of an image using the context information from the surroundings.
As the name implies, \textbf{colorization} task learns to color a grayscale input image, while \textbf{denoising} task learns to recover an image from a corrupted version.
\textbf{Models Genesis} aims to learn anatomical features of the body found consistently in a particular medical imaging protocol.
Following common practice in self-supervised learning, we evaluate our model in a transfer-learning experiment.
First, we train multiple networks using the pretext tasks mentioned above on the DRIVE dataset.
The trained networks are then \textit{finetuned} to learn the downstream supervised vessel segmentation task on the STARE dataset.
We consider a \textit{limited-data} scenario where only four images are provided for finetuning, and a \textit{high-data} scenario where finetuning is done with 16 images.
Figure \ref{fig:selfsupervised} shows the training dynamics in both the scenarios.
Our method takes very few iterations to converge compared to the other methods and achieves the best validation dice score.
Our results confirm that our design of self-supervised task is well-suited for the downstream vessel segmentation task.


\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{images/selfsupervised/highdata.png}
    \includegraphics[width=0.48\textwidth]{images/selfsupervised/lowdata.png}
    \caption{Validation curves on supervised vessel segmentation on STARE dataset with high data scenario (left) and limited data scenario (right). In both scenarios, our method achieves the best validation dice score much faster than the other self-supervision tasks.}
    \label{fig:selfsupervised}
\end{figure}

\subsection{COPDGene Dataset}


\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{images/COPD/COPDGene_1.pdf}
    \caption{Visualization of extracted vasculature in subject with minimal emphysema (top row) and severe emphysema (middle row). Red bounding box highlights vessel pruning in severe emphysema. The last row presents qualitative comparison with scale-space particles (SSP) based vessel-segmentation~\cite{estepar2012computational}.}
    \label{fig:COPD}
\end{figure}


% \subsection{Comparison with unsupervised methods}
% \subsubsection{DRIVE dataset}
% \begin{enumerate}
% \item We compare our method with other unsupervised vessel enhancement methods on the DRIVE dataset.
% \item Consists of 20 retinopathy images for training, and 20 for testing.
% \item To compute other metrics, use 5 ground truth images to find optimal threshold for all methods.
% \item Results are in Table 1.
% \item Our method produces better quality vessels and has lesser noise compared to Frangi because the other loss terms prevent over-fitting to local noise or artifacts.
% \end{enumerate}

% \subsubsection{VascuSynth dataset}
% \begin{enumerate}
% \item VascuSynth is a software for simulating volumetric images of vascular trees and generating the corresponding ground truth segmentations, bifurcation locations, branch properties, and tree hierarchy.
% \item They also provide a dataset for 10 groups, containing 12 volumes each.
% \item We use 6 groups for training, 1 for validation and 3 for testing. To check the robustness of our method, we augment the volumes with Gaussian noise with increasing values of $\sigma.$
% \item Results are in Table 4.
% \item Note that our method is more robust as the noise increases.  Adding a bifurcation term improves the metrics slightly, and there is a remarkable increase in dice scores and sensitivity.
% \end{enumerate}


% \subsection{Robust domain transfer}
% \begin{enumerate}
% \item Although our method cannot perform better than supervised methods out-of-the-box, we show that our method is more robust to domain shift.
% \item We train a supervised UNet on the DRIVE dataset. The performance on the DRIVE test set is more than any unsupervised method.
% \item However, testing the network on images from the STARE dataset shows that our method performs slightly better than supervised methods.
% \item We believe that this is because small errors in predicted radius and direction of the vessels do not lead to drastic change in vesselness scores.
% \end{enumerate}

% \subsection{Comparison with other self-supervised methods}
% \begin{enumerate}
%     \item To measure the effectiveness of our method as a self-supervised task, we train our method on the DRIVE dataset, and finetune with the STARE dataset.
%     \item We compare our method with two other self-supervised tasks, namely, context encoding, and denoising.
%     \item Training curves indicate that our method learns better feature representation that helps it converge faster in the downstream task.
% \end{enumerate}

% \subsection{Effect of test-time tracking score}
% \begin{enumerate}
% \item We also test the effect of augmenting the vesselness scores with the tracking based score described in Section ???.
% \item Results are in Table 2.
% \item It is easy to see that there are slight improvements in all metrics. The improvements are not that significant because the loss terms already handle the case of overfitting.
% \item Note that for each configuration of parameters, the metrics with and without test time tracking score augmentation are with the same network parameters.
% \end{enumerate}

% \subsection{Effect of bifurcation-based loss}
% \begin{enumerate}
% \item Normal metrics would not be able to show the improvement due to the bifurcation term because of the extreme sparsity of bifurcations (vessels are sparse in the image and bifurcations are sparse within vessels).
% \item We manually annotate bounding boxes centered around bifurcations in ground truth segmentation.
% \item For all methods, we compare the dice loss of the segmentation only in these bounding boxes.
% \item Results for all methods are shown in Table 3.
% \item We show that a lot of improvement comes from using the robust vessel metric. Moreover, the bifurcation-based vesselness metric shows an overall improvement in the dice score for bifurcations.
% \end{enumerate}


% \subsection{Ablation study of different loss functions}
% \begin{enumerate}
% \item Here we study the effect of setting different values of $\lambda_f, \lambda_i, \lambda_v$.
% \item Results are in Table 1.
% \item Using the voting based metric leads to more robust vesselness maps as compared to the cross-correlation based loss.
% \item Doesn't detect ridges and can thus detect low contrast vessels better.
% \item Qualitative results are in Figure ???.
% \end{enumerate}


==> sections/intro_v1.tex <==

\section{Introduction}
% We propose and formulate self-supervised loss functions for detection of tube-like structures in an image or volume.
% More specifically, we use generic properties of tubular structures to learn features to detect vessel-like structures in an unsupervised manner.
% Our goal is to use key properties of tubular structures to learn feature representations that can be used for unsupervised vessel enhancement, and can also be fine-tuned for a supervised vessel segmentation task with limited data.
% Our motivation comes from unsupervised multi-scale vessel enhancement algorithms, on which we provide a modern take using self-supervised learning. 
Tube-like structures, such as vessels and airways, are ubiquitous in human anatomy. 
Segmenting such structures is essential for characterizing the progression of many diseases~\cite{estepar2013computed}. Supervised deep learning methods have made significant progress for accurate segmentation, but large-scale annotated datasets are limited to 2D data and small sample size.
We develop a self-supervised that incorporates the structure's key properties and learn optimal representation for those.
Our method is applicable for both 2D and 3D, and it can be employed to bootstrap a supervised method in a semi-supervised setting. 

==> sections/method_v1.tex <==
%!TEX root = ../draft_v1.tex


\section{Method}
%This section describes the  method for a self-supervision task for vessel segmentation. 
%Figure \ref{fig:framework} describes the overall framework used for self-supervised learning.
%Our method takes an input image, which is fed into a fully-convolutional network (UNet for example) that outputs a vector field of vessel directions, the radius of the vessel at each voxel, and bifurcation angles at each voxel.
%These values are fed into various consistency loss functions that regularize the values of the vector field, vessel radius and bifurcation angles.
%Finally, these loss functions are added to form the final loss function for training.
%During testing, we use the outputs to perform scale-space vessel enhancement on the input image.
In this section, we introduce the overall framework for a self-supervised task for vessel enhancement.
Figure \ref{fig:framework} describes the overall schematic of our method.
Let $I$ be the input image.
This image is fed into a fully-convolutional network, denoted by $\mathcal{F}_\phi$, where $\phi$ are the parameters of the network.
The fully-convolutional network $\mathcal{F}_\phi$ outputs per-pixel parameters that characterize a vessel.
The first output is a vector field which is denoted by $u$ which signifies the direction of the vessel at each pixel.
We call this vector field the \textit{`vessel flow'} field.
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/frameworkv1.png}
    \caption{Overall framework of our method. The network $\mathcal{F}$ takes an image $I$ as input, and outputs vector and scalar fields that parameterize a vessel. The vector field is the direction of the vessel, and the scalar fields are the vessel radius, and bifurcation angles. The network is trained to produce correct parameters for these fields using various self-supervised loss functions.} 
    \label{fig:framework}
\end{figure}
The network $\mathcal{F}_\phi$ also outputs 3 scalar fields, namely $r$, $\theta_1$, and $\theta_2$ which signify the radius, and bifurcation half-angles respectively. 
The vector flow combined with the bifurcation half-angles result in two new vector fields denoted by $b_1$ and $b_2$, which are vector fields indicating the bifurcation directions.
These outputs can sufficiently characterize the presence of the vessel at each pixel.
To ensure that they characterize the vessel properly, these fields are passed onto various self-supervised and consistency loss functions, which we describe in the following sections. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Template alignment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Template alignment loss}
A vessel can be characterized by a tangent direction, and an associated radius.
To accommodate for varying thickness of the vessels, many unsupervised vessel enhancement methods \cite{unsup1} \cite{unsup2} apply their algorithm at multiple scales $s_1, s_2 \ldots s_n$.
However, the discrete nature of the chosen scales may limit the enhancement of intermediate sized vessels.
On the contrary, our method outputs a continuous scalar field $r$ which directly outputs the predicted vessel radius, allowing our method to work with continuous scales.
To align the vessel flow field and radius field, we take inspiration from template-matching based methods to match a fixed template with the image aligned using the outputs of the network.

\
e consider a fixed template $M$ which has a vessel of unit radius.
For a given point $p$, the image is spatially scaled using the radius $r(p)$ which resizes the vessel at point $p$ to have a unit radius.
Next, the image is rotated about the point $p$ such the $u(p)$ aligns with the template $M$.
We denote this transformation function as $T$ which takes as input the image $I$, the radius field $r$, the vessel flow field $u$, the pixel about which to apply the transformation $p$.
The output of the transformation function is also an image denoted by $T(I, r, u, p)$.
Finally, the similarity of the aligned image and the template $M$ is computed using Pearson's correlation coefficient (PCC) \cite{pcc}.
\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.9\textwidth]{images/alignment.png}
    \includegraphics[width=0.9\textwidth]{images/alignmentv1.png}
    \caption{Aligning the template with the image patch at point $p$. If the direction is correct but radius is too large (left image), the PCC of the patch and template is low. If the direction is not along the vessel tangent (right image), then the PCC is low as well. If the radius and direction are both correct (middle image), the PCC is maximized.}
    \label{fig:alignment}
\end{figure}
%The template alignment loss aligns the image patch such that it resembles a fixed vessel template given by $M$.
%At point $p$, the image patch should roughly look like a vessel along the direction $u(p)$ with respect to a given template $M$.
%To account for varying thickness of the vessel, we output a radius field $r$, where $r(p)$ is the predicted radius of the vessel at point $p$.
%The image is first spatially scaled using the radius $r(p)$ which makes the vessel from thickness $r(p)$ to a unit thickness.
%Next, the image patch is rotated about $p$ using $u(p)$ to orient the vessel along the image patch at $p$.
%Finally, we measure the similarity of the aligned image patch around $p$ and the template of unit vessel width $M$ using Pearson correlation coefficient (PCC).
%PCC allows us to account for changing contrast of the vessel, therefore allowing the loss not to be skewed by high-contrast regions.
A pictorial depiction is shown in Figure \ref{fig:alignment}. 

The template alignment loss for a pixel $p$ is simply:
\[
L_a(p) = 1 - \text{PCC}(M, T(I, r, u, p))
\]
The vesselness score can be formulated as:
\begin{align}
V(p) =  \text{CC}(M, T(I, r, u, p))
\label{eq:vesselness}
\end{align}
where CC is the correlation function. 
The choice of functions for the loss function and vesselness score is different because using Pearson's correlation coefficient will have the unintended side effect of amplifying noise and very low-contrast artifacts.
However, using the correlation function as a loss function will skew the loss towards high-contrast regions only.
This loss function ensures that $r$ and $u$ are trained to detect as many vessels as possible.
Next, we discuss other self-supervised loss functions that help regularize the values of the output vector fields and reduce overfitting.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Flow consistency
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Vector flow consistency loss}
The template alignment loss aligns the values of the radius and direction at each pixel to match with the best possible vessel.
However, there is a sign ambiguity in the vessel flow field.
Specifically, consider a point $p$ for which the vessel flow $u(p)$ points in the direction of the vessel.
Now consider a point in the neighborhood of $p$ along $u(p)$ at a distance $s$. 
The pixel location is given as $p + su(p)$.
Since the two points are close, the vessel direction should roughly be the same.
However, the vector flow $u(p + su(p))$ can point in the opposite direction of $u(p)$.
%Specifically, the vector $u(p)$ can point to the vessel direction at $p$, but the vessel direction in a neighbourhood point of $p$, say $q$ can point in the opposite direction without changing the template alignment loss.
Although this is a valid vessel flow field, the flow field can be discontinuous arbitrarily which doesn't lend itself to interpretation of the flow field.
Furthermore, penalizing discontinuity in the vessel flow field is a useful prior and can be an additional learning signal to learn faster.
%This makes the flow discontinuous which is slightly difficult to interpret, and may be harder to learn without an additional signal.
%Encouraging the nearby flow vectors to point in roughly the same direction is a reasonable prior that provides the network an additional learning signal.
\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.9\textwidth]{images/flow.png}
    \caption{
    %Depiction of the flow consistency loss. Note that for a small scalar $s$, the vessel direction $u(p + su(p))$ can point in the opposite direction of $u(p)$ and still have a low value of $L_a(p)$. However, we encourage the vectors to align along the vessel in the same direction as a useful prior.
    Depiction of the flow consistency loss. Given a point $p$, the vessel flow $u(p)$ points in the direction of the vessel.  However, at a neighborhood point, the vessel flow $u(p + su(p))$ can point in the opposite direction without affecting the template alignment loss.
    }
    \label{fig:flow}
\end{figure}
%To do that, we assume that vessel segments are locally straight lines in the scale-space, and their direction vectors $u$ should point in the same direction. 
Under the prior that the vessel flow doesn't change direction abruptly along the vessel, we propose the following loss function:
%We propose the loss function:
$$L_{f}(p) = 1 - \frac{\int_{0}^{2r(p)} \left< u(p), u(p + s\cdot u(p)))\right> ds}{\int_{0}^{2r(p)} ds}$$
This line integral encourages the flow vectors around $p$ to align in roughly the same direction. A pictorial depiction is shown in Figure \ref{fig:flow}.
So far, we have aligned the vessel flow field along vessels and ensured smoothness of the vessel flow field.
However, there can be noisy artifacts that the network may inadvertently consider as vessels and output a high template matching score for those pixels.  
In the next subsection, we propose loss functions to address this problem.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Vessel directions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Vesselness and intensity consistency loss}
%The previous loss functions ensure that the output fields are aligned correctly, and the vessel flow field is continuous along vessel directions.
%However, the image can have noisy regions or artifacts which the network can interpret as vessel structures.
%In these cases, the direction vectors can overfit to noisy regions which look like vessels to maximize the PCC for a given location.
%To regularize, we also encourage the vesselness and intensity to not change along the direction of the vessel.
%The idea is that for consistent vessels, this loss does not add an extra signal.
%However, for a region with local artifacts, it is difficult to match the intensity with any other point in its neighborhood due to the inconsistency in its neighborhood.
%Therefore, the radius parameter $r(p)$ in those pixels will shrink for the intensities to match.
In addition to a vessel tree, an image may contain other artifacts which can get high responses from the template.
However, a distinguishing factor between a vessel and other such structures is that the intensities are roughly the same along the vessel.
Similarly, the predicted vesselness are going to be roughly the same along the vessel.
To encode this property of vessel structures, we propose the following loss functions:

$$L_{v}(p) = \frac{\int_{0}^{2r(p)} \left( V(p + s u(p)) - V(p) \right)^2  ds}{\int_{0}^{2r(p)} ds}$$

$$L_{i}(p) = \frac{\int_{0}^{2r(p)} \left( I(p + s u(p)) - I(p) \right)^2  ds}{\int_{0}^{2r(p)} ds}$$

where $V$ is defined in Equation \ref{eq:vesselness} and $I$ is the input image. It is depicted pictorially in Figure \ref{fig:icvc}.
The loss functions take the average intensity error and average vesselness error along the predicted vessel.
Correctly predicted vessels will have a low error because the intensity and vesselness are locally the same along the vessel.
For a noisy pixel $r$, the only way to minimize these errors is to make $r$ close to 0 because the intensity will be the same at the sub-pixel level.
In our experiments, we show that adding these loss terms improves the overall prediction of vessels.

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{images/ic.png}
    \caption{Pictorial depiction of Intensity consistency loss (vesselness consistency loss is defined similarly where $I$ is replaced with $V$). Note that the intensities do not change along the vessel, but in regions with vessel-like artifacts, it is difficult to match intensities with a neighbourhood.}
    \label{fig:icvc}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Robustness of metric
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Robust vesselness metric}
In spite of all these losses, a common bottleneck in most unsupervised methods is the vesselness metric itself.
Many unsupervised methods cannot distinguish between a low-contrast vessel and a high-intensity ridge.
This applies to Hessian-based methods, gradient-based methods, and template based methods as well. 
The reason is that ridges look like vessels from one direction, therefore ridges get a partial match from these methods.
However, the key insight is that ridges look like vessels, but only from one direction.
%We use this to formulate our vesselness metrics, which we name ``mPCC'' and ``mCC'' (replacements of the PCC and CC metrics respectively).
We use this insight to replace the PCC and CC metrics with our proposed metrics which we name ``mPCC'' and ``mCC'' respectively.
The mPCC metric works by taking several ``half-templates'' and computing the PCC of the image with each of the half-templates.
The final response is simply the minimum of these responses.
Mathematically, if $M_1, M_2 \ldots M_K$ are $K$ ``half-templates'' and $I$ is the input image, the metric is:
$$
 \text{mPCC}(I, M_1, \ldots M_K) = \min_{k=1}^{K} PCC(I, M_k)
$$
The corresponding vesselness metric ``mCC'' is also defined similarly.
$$
 \text{mCC}(I, M_1, \ldots M_K) = \min_{k=1}^{K} CC(I, M_k)
$$
An example of robustness of ``mCC'' for 2D is shown in Figure \ref{fig:robustvesselness}.
More details about the metric is provided in the Appendix.
\begin{figure}[htpb]
    \centering
    \includegraphics[width=\textwidth]{images/cc.png}
    \includegraphics[width=\textwidth]{images/mcc.png}
    \caption{A comparison of cross-correlation (CC) and our robust metric mCC. The top figure shows the output of cross-correlation of the image and the template, which has a same response to both the low-contrast vessel and the high-contrast ridge. On the contrary, our propsed vesselness metric (bottom) uses 2 half templates for 2D, and the minimum response vanishes for the ridge because one ``half-template'' does not match with the ridge at all.}
    \label{fig:robustvesselness}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Bifurcation aware loss
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bifurcation-aware loss}
So far, we have only considered vessels that are locally straight lines, and their scale and orientation is predicted by our network.
However, these parameters are insufficient to parameterize a bifurcation.
To accomodate the presence of bifurcations, we add two new outputs - the half-angle maps for bifurcations $\theta_1, \theta_2$.
The vector $-u(p)$ is rotated by $\theta_1(p)$ and $\theta_2(p)$ to get branch directions $b_1(p)$ and $b_2(p)$.
% The half-angles are constrained from 0 to $\frac{\pi}{2}$ to avoid degenerate cases like the half-angle being equal to $\pi$ which may ignore a real bifurcation happening.
The half-angles are constrained to avoid degenerate cases like the half-angle being equal to $\pi$ which may ignore a real bifurcation.
If there is no bifurcation, the half-angles simply become 0 which indicates a vessel without bifurcations.
An example of how the bifurcation loss works is shown in Figure \ref{fig:bifurc}.

\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\textwidth]{images/bifurc.png}
    \caption{An example of how bifurcation directions change for a point where bifurcation is absent (left) and when bifurcation is present (right).}
    \label{fig:bifurc}
\end{figure}

Mathematically, given the vector $u(p)$ and half-angles $\theta_1(p), \theta_2(p)$, we we obtain $b_1(p), b_2(p)$.
The template is matched for all 3 directions using:
$$
R(p) = \text{PCC}(M, T(I, p, r, u))
$$
$$
R_{b1}(p) = \text{PCC}(M, T(I, p, r, b_1))
$$
$$
R_{b2}(p) = \text{PCC}(M, T(I, p, r, b_2))
$$
$$
L_b(p) = 1 - \frac{R(p) + R_{b1}(p) + R_{b2}(p)}{3}
$$
For 3D images, we output $b_1(p)$ and $b_2(p)$ directly.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Test-time post-processing  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Test time post-processing using tracking}
During test time, we want to further dampen the vesselness metric there are small segments disconnected from the larger vessel structure.
This helps in dampening the response from local artifacts or noisy patches, while keeping the response from connected vessels intact.
We augment the vesselness metric with a tracking-based score in the scale space.
Intuitively, we want to see if the vessel flow changes its direction within an extended scale-space neighbourhood along the vessel.
To this end, we propose the following score:
$$
V_{t}(p) = \frac{\int_{0}^{4r(p)} | \left< u(p), u(p + s\cdot u(p))\right> | \quad ds}{\int_{0}^{4r(p)} ds}
$$
Note that this integral is over a larger scale-space neighborhood than the loss functions used in training.
This is done to prevent this score to be robust to overfitting over the smaller scale-space neighborhood from the training losses.
Given the tracking-based score, we augment our vesselness metric as such:
$$
U(p) = V(p) \cdot V_t(p)  
$$
This dampens the vesselness score where the vessels are not consistent in the extended scale-space neighborhood. 



==> sections/method_v2.tex <==
%!TEX root = ../draft_v1.tex

\section{Method}

This section will use some of the key properties of \emph{tube-like} structures (\eg vessels) to define a self-supervised algorithm. We use vessel structure as a running example, but the proposed method is general and can be applied to other tube-like structures such as airways. We consider three properties: (1) Profile Symmetry, (2) Path continuity, and (3) Possible bifurcation:

\begin{enumerate}
    \item The definition of \emph{profile symmetry} is dependent on the vessel flow. An orthogonal profile of the vessel's flow should be radially symmetric around the axis defined by the flow. In other words, the orthogonal profile of the tube structure can be approximated by a predefined template, $T$. For a vessel, the $T$ is simply a unit circle.
    
    \item The \emph{path continuity} assumes that the vessel trees' structure and arrangement can be viewed as a continuous path in space. We represent the path by a \emph{vector field}, where at each point inside the vessel, the vectors field's directions are aligned with the vessel's directionality. We refer to the vector field as \emph{vessel flow} field.
    
    \item Finally, the \emph{possible bifurcation} refers to the fact that the vessel may bifurcate. We use two vector fields to model the bifurcation. Wherever there is a bifurcation, the two vector fields point toward each bifurcation branch; otherwise, they are aligned with the vessel flow.
\end{enumerate}
  The idea has been shown in \figurename{\ref{fig:framework}}. We define the losses to enforce those properties. 

%In addition to this formulation, we also propose a few regularization loss functions which enforce other consistencies of the tube-like structures.
%For example, the intensity of the vessels should not change drastically along the vessel flow.
%Using these properties, we also define a vesselness metric which is robust to other structures that are similar to tubular structures, like flat ridges.

\textbf{Notation:}
Let $I: \Omega \rightarrow \mathbb{R}$ be the input image, where $\Omega \subset \sR^d$ is the domain of the input image, and $d$ is the dimensionality of the image.
For our paper, we consider $d \in \{2, 3\}$.
Let $\vu : \Omega \to \sS^{d-1}$ be used to denote the vessel flow where $\sS^{d-1}$ is the $d$-dimensional unit hypersphere.
Similar to the vessel flow, we also define two flows $\vb_1: \Omega \rightarrow \sS^{d-1}$ and $\vb_2: \Omega \rightarrow \sS^{d-1}$ which represent the two directions of the bifurcation.
Furthermore, we define a scalar field $r: \Omega \to \sR^{+} $ defining the radius of the tube.
We use $T: \Omega \rightarrow \sR$ to denote a canonical template for the tube-like structure of unit radius.
Finally, we use $\Phi_\theta: \Omega \to \Omega$ to define a transformation function parameterized by $\theta = (r, \vu)$.
\begin{figure}[htpb]
    \centering
    \includegraphics[width=\textwidth]{images/frameworkv2.pdf}
    \caption{Overall framework of our method} 
    \label{fig:framework}
\end{figure}
%We are going to use $I: \Omega \rightarrow \mathbb{R}$ to denote input image where $\Omega \subset \sR^d$ is the input domain and $d$ is the dimensionality of the image. We $\vu : \Omega \rightarrow \sS^{d-1}$ to denote the tube-flow where $\sS^{d-1}$ denotes unit hypersphere of embedded in $d$-dimensional space. For the bifurcation, we define two more flows $\vb_1: \Omega \rightarrow \sS^{d-1}$ and $\vb_2 : \Omega \rightarrow \sS^{d-1}$ each representing the directionality of the birfurcation. Furthermore, we define a scalar field $r: \Omega \rightarrow \sR^{+}$ defining the radius of the tube. We use $T: \Omega \rightarrow \sR$ to denote protypical template for the tube-like structure. We use $\Phi_{\theta}: \Omega \rightarrow \Omega $ is a transformation parametrized by $\theta$.

We now describe each of the self-supervised loss functions in the following subsections.

%%% Profile symmetry 
\subsection{Profile symmetry}
To determine the radius of the tube, we locally match the profile of the tube with a canonical template of a tube with unit radius.
At the given point $\vp \in \Omega$, we apply an affine transformation $\Phi_{\theta_\vp}$ parameterized by $\theta_\vp = (r(\vp), \vu(\vp))$ on the template $T: \Omega \rightarrow \mathbb{R}$.
The affine transformation works by first spatially scaling the template by $r(\vp)$. 
This modifies the canonical template to now have a tube from unit radius to a radius of $r(\vp)$.
Next, the affine transformation rotates the template such that the tube in the template aligns with the direction $\vu(\vp)$.
If $r(\vp)$ and $\vu(\vp)$ are predicted accurately, then the local vessel at $\vp$ will align with the modified template $T \circ \Phi_{\theta_\vp}(\vp)$.
The degree of alignment can be measured by a similarity metric $S: \Omega \times \Omega \to \sR$.
Hence, $r(\vp)$ and $\vu(\vp)$ should be set to values that maximize
$ S (I, T \circ \Phi_{r(\vp), \vu(\vp)}(\vp) )$.
In our case, we choose Pearson's correlation coefficient as the similarity metric.
Therefore, for a point $\vp$, the loss function for aligning the radius and flow can be written as:
\begin{equation}
    \mathcal{L}_a(\vp) = 1 - S (I, T \circ \Phi_{\theta_p}(\vp) )
    \label{eq:alignment}
\end{equation}
To minimize this loss function, the similarity must be maximum which implies $r(\vp)$ and $\vu(\vp)$ must be predicted accurately.

\subsubsection{Vesselness metric}
Given a prediction of $r(\vp)$ and $\vu(\vp)$, we also compute a ``vesselness'' metric and a corresponding function.
This metric is denoted by $\mathcal{V}: \Omega \times \Omega \to \sR$ and the function is given as $V: \Omega \to \sR$. 
In our case, we choose $\mathcal{V}$ to be the cross-correlation metric. 
Given an image $I$, a point $\vp$, and the radius and vessel flow fields, the vesselness of the point $\vp$ is defined as $V(\vp) = \mathcal{V}(I, T \circ \Phi_{\theta_\vp}(\vp))$.

%%% Path continuity
\subsection{Path Continuity}
The symmetry of the canonical template along the tube leads to a sign ambiguity in the vessel flow, which may cause discontinuities in the vessel flow field.
This is because reversing the direction of the tube does not change the template, which means for a point $\vp$, $\vu(\vp)$ and $-\vu(\vp)$ will result in the same similarity value.
To break the sign ambiguity, we propose a loss function to encourage the vessel flow to be in the same direction along the vessel.
% This provides an additional learning signal while encouraging the continuity of the vessel flow field along the tube-like structure.
%To formulate the loss, consider $T$ positive, equally spaced step sizes $s_1 \le s_2 \ldots \le s_T$ along the vessel for which we want to ensure the alignment of the vessel flow.
%For a step size $s_t$, the point after moving from $\vp$ along the vessel flow $\vu(\vp)$ is simply $\vq(s_t) = \vp + s_t\vu(\vp)$.
To formulate the loss, consider starting from a location $\vl_\vp(0) = \vp$ and moving to a location $\vl_\vp(s)$ by taking small steps of length $\Delta s$, and adding up the alignment losses at locations $\vl_\vp(s)$.
If we move from the current location $\vl_\vp(s)$ to the next point $\vl_\vp(s + \Delta s)$, the 2 locations are related by the following equation:
$$
\vl_\vp(s + \Delta s) = \vl_\vp(s) + \Delta s\cdot \vu(\vp)
$$
because the step sizes are taken along the vessel direction $\vu(\vp)$.
Taking the limit $\Delta s \to 0$, we can write this equation as:
\begin{equation}
    \frac{d \vl_\vp(s)}{ds} = \vu(\vp)
    \label{eq:deltal}
\end{equation}
Now, we need a metric that measures the degree of alignment between the vessel flow at $\vp$ and vessel flow at $\vq$.
For our paper, we choose the cosine similarity or dot product of the vessel flow at these locations (since both vectors are of unit magnitude):
$
\left< \vu(\vp), \vu(\vq) \right> 
$.
We need to maximize this alignment for all locations $\vl_\vp(s)$.
%If the alignment loss after considering step-sizes upto $\mathcal{L}_f(\vp, t)$, the alignment loss after considering $t+1$ step-sizes is:
If the alignment loss after considering locations till $\vl_\vp(s)$ is $\mathcal{L}_f(\vp, s)$, then the alignment loss after considering locations till $\vl_\vp(s + \Delta s)$ is:
\begin{equation}
%\mathcal{L}_f(\vp, t+1) = \mathcal{L}_f(\vp, t) - \left< \vu(\vp), \vu(\vp + s_{t+1} \vu(\vp)) \right>
\mathcal{L}_f(\vp, s + \Delta s) = \mathcal{L}_f(\vp, s) - \left< \vu(\vl_\vp(0)), \vu(\vl_\vp(s)) \right> \Delta s
\label{eq:cosinediscrete}
\end{equation}
%In the limiting case when $T \to \infty$ and $s_{t+1} - s_{t} = d s$, Equation {\ref{eq:cosinediscrete}} becomes:
In the limiting case when $\Delta s \to 0$, Equation \ref{eq:cosinediscrete} becomes:
\begin{equation}
%\frac{d \mathcal{L}_f(\vp, t)}{d t} = -\left< \vu(\vp), \vu(\vp + s(t)\vu(\vp)) \right>
\frac{d \mathcal{L}_f(\vp, s)}{d s} = -\left< \vu(\vl_\vp(0)), \vu(\vl_\vp(s)) \right>
\label{eq:odecos}
\end{equation}
%Since $s(t)$ is linearly related to $t$ from our formulation, using a change of variables, we get:
%\begin{equation}
%\frac{d \mathcal{L}_f(\vp, s)}{d s} = -\left< \vu(\vp), \vu(\vp + s\vu(\vp)) \right>
%\label{eq:odecos}
%\end{equation}
Starting from an initial value $\mathcal{L}_f(\vp, 0) = 0$ and $\vl_\vp(0) = \vp$, we define our final alignment loss as $\mathcal{L}_f(\vp)$ which is the integral of the Equation \ref{eq:odecos}.
To solve for Equation \ref{eq:odecos}, we solve Equation \ref{eq:odecos} and \ref{eq:deltal} simultaneously using the integral:
%which is solved as:  % $\mathcal{L}_f() = \mathcal{L}_f(\vp, 2r(\vp))$ which is the solution of Equation \ref{eq:odecos}.
\begin{equation}
    \begin{bmatrix}
    \mathcal{L}_f(\vp) \\
    \vl_\vp \\
    \end{bmatrix}
    = 
    \begin{bmatrix}
    0 \\ \vp 
    \end{bmatrix} + 
    \int_0^{2r(\vp)} \begin{bmatrix}
    -\left< \vu(\vl_\vp(0)), \vu(\vl_\vp(s)) \right> \\
    \vu(\vp) \\
    \end{bmatrix} ds
    \label{eq:bigodecos}
\end{equation}
where $\mathcal{L}_f(\vp)$ is shorthand notation for $\mathcal{L}_f(\vp, 2r(\vp))$ and $\vl_\vp$ is short for $\vl_\vp(2r(\vp))$.
Equation \ref{eq:bigodecos} can be solved using a differentiable ODE solver.
%Note that the second argument to $\mathcal{L}_f$ is equal to $2r(\vp)$ (instead of being a constant) to ensure that larger line segments are considered for larger tube-like structures and similarly for smaller line segments.
Note that the upper limit in the integral is $2r(\vp)$ instead of being a constant to ensure that larger line segments are considered for larger vessels, and similarly for smaller vessels.
Next, we describe a loss function to detect the presence of bifurcation angles, and use the existing template alignment idea to predict the bifurcation flow fields. 
%%% Bifurcations
\subsection{Predicting bifurcations}
The bifurcation flow fields $\vb_1$ and $\vb_2$ can be predicted in a similar way to the vessel flow.
Consider a point $\vp$, where a vessel arriving from the direction $-\vu(\vp)$ splits into two vessels along directions $\vb_1(\vp)$ and $\vb_2(\vp)$.
%Therefore, the region starting from $\vp$ along $-\vu(\vp)$ should look like a tube, and the region  
In this case, the region centered around $\vp$ does not resemble the template. % , and $S(I, T \circ \Phi_{\theta_\vp}(\vp))$ will be low.
However, the region starting from $\vp$ along $\vu(\vp)$ should look like a tube since $\vp$ is the point where the tube bifurcates.
After the bifurcation, the region starting from $\vp$ along $\vb_1(\vp)$ should also resemble a vessel, because after the bifurcation, two new vessels start in new directions.
The same argument holds for $\vb_2(\vp)$ as well.
Therefore, the bifurcation loss finds the radius, vessel flow and bifurcation flow fields $r, \vu, \vb_1, \vb_2$ to maximize the similarity of the canonical template to the incoming vessel, and the two branched vessels.
Similar to Equation \ref{eq:alignment}, we calculate the similarities to the 3 segments $S(I, T \circ \Phi_{\{r(\vp), \vv(\vp)\}}(\vp))$ where $\vv(\vp) \in \{ \vu(\vp), \vb_1(\vp), \vb_2(\vp) \}$, and therefore, the loss is written as:

\begin{equation}
    \mathcal{L}_b(\vp) = 1 - \frac{\sum_{\vv(\vp) \in \{ \vu(\vp), \vb_1(\vp), \vb_2(\vp) \}} S(I, T \circ \Phi_{\{r(\vp), \vv(\vp)\}}(\vp)) }{3}
    \label{eq:bifurc}
\end{equation}

Note that if there is no bifurcation, then $\vb_1(\vp) = \vb_2(\vp) = -\vu(\vp)$ minimizes the loss function.
Since the loss encapsulates the case when there is no bifurcation, we can replace the loss function in Equation \ref{eq:alignment} with Equation \ref{eq:bifurc}.

The neural network is parameterized such that bifurcation flow fields $\vb_1$ and $\vb_2$ always satisfy $\left< \vb_1(\vp), \vu(\vp) \right> \le 0$ and $\left< \vb_2(\vp), \vu(\vp) \right> \le 0$ for all $\vp \in \Omega$.
This is done to prevent the bifurcation directions and vessel flow from collapsing into one single direction.

\subsection{Intensity and vesselness consistency losses}
Without the ground truth, the network finds the radius and vessel flow fields that maximize the similarity of the image and the template at every pixel.
In a typical image however, there may be many other artifacts which can have a high similarity with the template.
But there is a key property that the tube-like structures satisfy which other artifacts may not satisfy.
Locally, the image intensities along the vessel are roughly equal, but for noise or artifacts, the image intensities will vary rapidly.
Inspired by this idea, we propose a regularization loss that computes the intensity error along the vessel. 
%Similar to before, we take $T$ positive, equally spaced step sizes $s_1 \le s_2 \ldots \le s_T$ for which we want to measure the intensity error.
%If the intensity error after considering $t$ step sizes is $\mathcal{L}_i(\vp, t)$, the alignment loss after considering $t+1$ step sizes is:
%$$ 
%\mathcal{L}_i(\vp, t+1) = \mathcal{L}_i(\vp, t) + \left[ I(\vp) - I(\vp + s_{t+1}\vu(\vp)) \right]^2
%$$
Similar to the formulation for path continuity, we start from the location $\vl_\vp(0) = \vp$ and move to a location $\vl_\vp(s)$ along $\vu(\vp)$ using steps of size $\Delta s$.
The dynamics of $\vl_\vp(s)$ is given in Equation \ref{eq:deltal}.
Now, if the intensity error after considering locations till $\vl_\vp(s)$ is denoted by $\mathcal{L}_i(\vp, s)$, the alignment loss after considering locations till $\vl_\vp(s + \Delta s)$ is:
\begin{equation}
\mathcal{L}_i(\vp, s + \Delta s) = \mathcal{L}_i(\vp, s) + \| I(\vl_\vp(s)) - I(\vl_\vp(s + \Delta s)) \|_2 
\label{eq:discreteli}
\end{equation}
Since $\Delta s$ is small and $\vl_\vp(s + \Delta s) = \vl_\vp(s) + \Delta s\cdot \vu(\vp)$, the right hand side of the equation can be written as
$$
I(\vl_\vp(s + \Delta s)) = I(\vl_\vp(s)) + \nabla I(\vl_\vp(s))^T \vu(\vp) \Delta s 
$$
where $\nabla I$ is the gradient of the image. 
Subsituting this equation and taking the limit $\Delta s \to 0$ in Equation \ref{eq:discreteli}, we get:
\begin{equation}
    \frac{d \mathcal{L}_i(\vp, s)}{ds} = \Big \| \nabla I(\vl_\vp(s))^T \vu(\vp) \Big\|_2
    \label{eq:odei}
\end{equation}
Similarly, for minimizing the vesselness error $V$ along the vessel flow, we formulate a similar differential equation for the loss function $\mathcal{L}_v(\vp, s)$ given by:
\begin{equation}
\frac{d \mathcal{L}_v(\vp, s)}{ds} = \Big \| \nabla V(\vl_\vp(s))^T \vu(\vp) \Big\|_2
\label{eq:odev}
\end{equation}
To solve for Equation \ref{eq:odei} and \ref{eq:odev}, we simultaneously solve the equations using:
\begin{equation}
   \begin{bmatrix}
   \mathcal{L}_i(\vp) \\
   \mathcal{L}_v(\vp) \\
   \vl_\vp \\
   \end{bmatrix} 
   = \begin{bmatrix}
   0 \\ 0 \\ \vp 
   \end{bmatrix} + 
   \bigints_0^{2r(\vp)} \begin{bmatrix}
   \Big \| \nabla I(\vl_\vp(s))^T \vu(\vp) \Big \| \\ 
   \Big \| \nabla V(\vl_\vp(s))^T \vu(\vp) \Big \| \\
   \vu(\vp)
   \end{bmatrix} ds
\end{equation}
where $\mathcal{L}_i(\vp)$ and $\mathcal{L}_v(\vp)$ are shorthand notations for $\mathcal{L}_i(\vp, 2r(\vp))$ and $\mathcal{L}_v(\vp, 2r(\vp))$ respectively.
The integrals can be computed using a differentiable ODE solver.
The reasoning for choice of upper limit in the integral is the same as that of the path continuity loss.

%Similar to Equation \ref{eq:cosinediscrete}, we take this equation to the limiting case and after a change of variables like before, we get:
%\begin{equation}
    %\frac{d \mathcal{L}_i(\vp, s)}{ds} = \left[ I(\vp) - I(\vp  + s\vu(\vp)) \right]^2
%\end{equation}
%We can solve this ODE with the initial value $\mathcal{L}_i(\vp, 0) = 0, \mathcal{L}_v(\vp, 0) = 0, \vl_\vp(0) = \vp$ to get the intensity error along the vessel flow segment which is equal to $\mathcal{L}_i(\vp, 2r(\vp))$. \\
%We can use a similar idea to take the error of the vesselness function along the vessel flow segment as well.
%This is due to the assumption that the tube-like structures are continuous and therefore do not change their contrast drastically along the tube.
%If this error is measured by $\mathcal{L}_v(\vp, s)$, it satisfies the ODE:
%\begin{equation}
    %\frac{d \mathcal{L}_v(\vp, s)}{ds} = \left[ V(\vp) - V(\vp  + s\vu(\vp)) \right]^2
%\end{equation}
%We compute the total vesselness error along the vessel flow segment which is given by $\mathcal{L}_v(\vp, 2r(\vp))$.



\subsection{Robust vesselness metric}
The primary caveat of commonly used vesselness functions is that they also have a high response to other structures that are geometrically very different from tubular structures.
One such example is a ridge, which is usually indicative of a flat surface.
Although a ridge is very different from a vessel, commonly used vesselness functions \cite{unsup} \cite{unsup} \cite{unsup} 

\subsection{Postprocessing}

%aq* We are going to define some of the properties of the tube-like structures such as vessels to come up with a self-supervised algorithm.

%* (1) The first property is vessel continuity. The idea is that vessel can be viewed as continious path. We use a vector field which we call \emph{vessels flow}.

%* (2) The second property build on top of the first property. The flow characterize the directionality of the tube. Orthogonal profile with respect to the flow is radially symmetric around the axis defined by the flow.

%* (3) The third property the bifurcation possibility. For example, vessel have tree-like structure that include bifurcations. We also use the first property to model the bifurcation. We view bifurcation as splitting flow. The bifurcation is also modeled as a vector field which deviates from the vessel flow whereever we have bifurcation. 

%* Our formulation also has a few regularization enforcing other consistencies of the tube-like structure. For example, the intensity of the vessels should not change drastically if we walk along the vessel flow. 

%* The idea is shown in \figurename{\ref{fig:framework}}


%* We start the method section with explainign the second property followed by vessel-flow and formulation of the birfurcation. 

%\textbf{Notation:} 
%We are going to use $I: \Omega \rightarrow \mathbb{R}$ to denote input image where $\Omega \subset \sR^d$ is the input domain and $d$ is the dimensionality of the image. We $\vu : \Omega \rightarrow \sS^{d-1}$ to denote the tube-flow where $\sS^{d-1}$ denotes unit hypersphere of embedded in $d$-dimensional space. For the bifurcation, we define two more flows $\vb_1: \Omega \rightarrow \sS^{d-1}$ and $\vb_2 : \Omega \rightarrow \sS^{d-1}$ each representing the directionality of the birfurcation. Furthermore, we define a scalar field $r: \Omega \rightarrow \sR^{+}$ defining the radius of the tube. We use $T: \Omega \rightarrow \sR$ to denote protypical template for the tube-like structure. We use $\Phi_{\theta}: \Omega \rightarrow \Omega $ is a transformation parametrized by $\theta$.

%\subsection{Second Property}
%* To determine the radious of the tube, we locally match the profile of the tube with a canonical template. 

%* At the given point $p \in \Omega$, We apply an affine transformation $\Phi_{\theta}$ parameterized by $\theta$ on the template $T$ where the parameters are \emph{locally} specified by we do that by the vessel-flow $\vu$ and scale it locally with scalar radius $r$. 
%\begin{equation}
    %I(p) \approx T \circ \Phi_{(r(p),\vu(p) )} (p)
%\end{equation}


%\subsection{First Property}
%
%\subsection{Third Property}
%
%\subsection{Regularization}
%
%\subsection{Post Processing}


==> sections/method_v2_s.tex <==
%!TEX root = ../draft_v1.tex

\section{Method}

This section will use some of the key properties of \emph{tube-like} structures (\emph{e.g.,} vessels) to define a self-supervised algorithm. We use vessel structure as a running example, but the proposed method is general and can be applied to other tube-like structures such as airways. We consider the following three properties,

\begin{itemize}
    \item \textbf{Path continuity}: The path continuity assumes that the vessel trees' structure and arrangement can be viewed as a continuous path in space. We represent the path by a \emph{vector field}, where at each point inside the vessel, the vectors field's directions are aligned with the vessel's directionality. We refer to the vector field as \emph{vessel flow} field.

    \item \textbf{Profile symmetry}: The definition of profile symmetry is dependent on the vessel flow. An orthogonal profile of the vessel's flow should be radially symmetric around the axis defined by the flow. In other words, the orthogonal profile of the tube structure can be approximated by a predefined template, $T$. For a vessel, $T$ is simply a unit circle.
    
    
    \item \textbf{Bifurcation}: The possible bifurcation refers to the fact that the vessel may bifurcate. We use two vector fields to model the bifurcation. Wherever there is a bifurcation, the two vector fields point toward each bifurcation branch; otherwise, they are aligned with the vessel flow.
\end{itemize}
  The idea has been shown in \figurename{\ref{fig:framework}}. We define the losses to enforce those properties. 

%In addition to this formulation, we also propose a few regularization loss functions which enforce other consistencies of the tube-like structures.
%For example, the intensity of the vessels should not change drastically along the vessel flow.
%Using these properties, we also define a vesselness metric which is robust to other structures that are similar to tubular structures, like flat ridges.

\textbf{Notation:}
Let $I: \Omega \rightarrow \mathbb{R}, \Omega \subseteq \sR^d$ be the $d$-dimensional image. We consider $d \in \{2, 3\}$.
Let $\vu : \Omega \to \sS^{d-1}$ denote  the vessel flow, defined as a vector field where for any point $p \in \Omega$, $\sS^{d-1}$ is a $d$-dimensional unit hypersphere centered at $p$.
We define $\vb_1: \Omega \rightarrow \sS^{d-1}$ and $\vb_2: \Omega \rightarrow \sS^{d-1}$ to represent the two directions of the bifurcation.
Furthermore, $r: \Omega \to \sR^{+} $ is defined as a scalar field to represent the radius of the vessel.
We use $T: \Omega \rightarrow \sR$ to denote a canonical template for the tube-like structure of unit radius.
Finally, we use $\Phi_\theta: \Omega \to \Omega$ to define a transformation function parameterized by $\theta = (r, \vu)$.
\begin{figure}[htpb]
    \centering
    \includegraphics[width=\textwidth]{images/frameworkv2.pdf}
    \caption{Overall framework of our method} 
    \label{fig:framework}
\end{figure}
%We are going to use $I: \Omega \rightarrow \mathbb{R}$ to denote input image where $\Omega \subset \sR^d$ is the input domain and $d$ is the dimensionality of the image. We $\vu : \Omega \rightarrow \sS^{d-1}$ to denote the tube-flow where $\sS^{d-1}$ denotes unit hypersphere of embedded in $d$-dimensional space. For the bifurcation, we define two more flows $\vb_1: \Omega \rightarrow \sS^{d-1}$ and $\vb_2 : \Omega \rightarrow \sS^{d-1}$ each representing the directionality of the birfurcation. Furthermore, we define a scalar field $r: \Omega \rightarrow \sR^{+}$ defining the radius of the tube. We use $T: \Omega \rightarrow \sR$ to denote protypical template for the tube-like structure. We use $\Phi_{\theta}: \Omega \rightarrow \Omega $ is a transformation parametrized by $\theta$.

%We now describe each of the self-supervised loss functions in the following subsections.
We first explain the profile symmetry followed by path continuity and bifurcation.

%%% Profile symmetry 
\subsection{Profile symmetry}
We defined the profile of a vessel point  $\vp \in \Omega$  in-terms of its radius $r(\vp)$ and direction of flow $\vu(\vp)$.
To determine the profile, we locally matched each vessel point $\vp$ with a canonical template of a tube ($T$). We achieved this matching by applying  an affine transformation $\Phi_{\theta_\vp}$, parameterized by $\theta_\vp = (r(\vp), \vu(\vp))$, on the template $T$.
The affine transformation spatially scales $T$ to have  a radius of $r(\vp)$, followed by a rotation to align $T$  with the direction of flow $\vu(\vp)$.
If the profile is predicted accurately, then the local vessel at $\vp$ will align with the modified template $T \circ \Phi_{\theta_\vp}(\vp)$.
We measured the degree of alignment as a similarity metric $S: \Omega \times \Omega \to \sR$ between the raw image $I$ and the modified template. To maximize the similarity metric and thus find an accurate profile for a vessel point $\vp$, we minimize the following loss function,
\begin{equation}
    \mathcal{L}_a(\vp) = 1 - S(I, T \circ \Phi_{r(\vp), \vu(\vp)}(\vp)  )
    \label{eq:alignment}
\end{equation}
Here, we employed Pearson's correlation coefficient as the similarity metric.

\subsubsection{Vesselness metric}
Given the predicted profile $\{r(\vp), \vu(\vp)\}$, we also compute a ``vesselness'' metric denoted by $\mathcal{V}: \Omega \times \Omega \to \sR$ and defined as $V(\vp) = \mathcal{V}(I, T \circ \Phi_{\theta_\vp}(\vp))$. For our experiments,  we choose $\mathcal{V}$ to be the cross-correlation metric. 

%%% Path continuity
\subsection{Path continuity}
The template T is symmetric with respect to the direction of a vessel. Hence, for a point $\vp$, $\vu(\vp)$ and $-\vu(\vp)$ will result in the same similarity value ($S(\vp)$). This symmetry may lead to sign ambiguity in the vessel flow $\vu$, resulting in discontinuities in $\vu$.
To prevent such ambiguity, we propose an alignment loss  that encourages $\vu$ to have a consistent direction along the vessel.
% This provides an additional learning signal while encouraging the continuity of the vessel flow field along the tube-like structure.
%To formulate the loss, consider $T$ positive, equally spaced step sizes $s_1 \le s_2 \ldots \le s_T$ along the vessel for which we want to ensure the alignment of the vessel flow.
%For a step size $s_t$, the point after moving from $\vp$ along the vessel flow $\vu(\vp)$ is simply $\vq(s_t) = \vp + s_t\vu(\vp)$.
To formulate the loss, we start from  point $\vp$, with location $\vl_\vp(0)$ and traverse along the direction of vessel flow \emph{i.e.,}  $\vu(\vp)$ while taking small steps of length $\Delta s$. Our traversal is defined as,
$$
\vl_\vp(s + \Delta s) = \vl_\vp(s) + \Delta s\cdot \vu(\vp)
$$
Taking the limit $\Delta s \to 0$, we can re-write this equation as:
\begin{equation}
    \frac{d \vl_\vp(s)}{ds} = \vu(\vp)
    \label{eq:deltal}
\end{equation}

We further used the cosine similarity metric $\left< \vu(\vp), \vu(\vq) \right> $, to measure the degree of alignment between vessel flow at any two points, $\vp$ and $\vq$.
To ensure path continuity, we maximize vessel flow alignment for all the points $\vl_\vp(s)$ on our traversal path.
%If the alignment loss after considering step-sizes upto $\mathcal{L}_f(\vp, t)$, the alignment loss after considering $t+1$ step-sizes is:
We incrementally learn the alignment loss as,
\begin{equation}
%\mathcal{L}_f(\vp, t+1) = \mathcal{L}_f(\vp, t) - \left< \vu(\vp), \vu(\vp + s_{t+1} \vu(\vp)) \right>
\mathcal{L}_f(\vp, s + \Delta s) = \mathcal{L}_f(\vp, s) - \left< \vu(\vl_\vp(0)), \vu(\vl_\vp(s)) \right> \Delta s
\label{eq:cosinediscrete}
\end{equation}
%In the limiting case when $T \to \infty$ and $s_{t+1} - s_{t} = d s$, Equation {\ref{eq:cosinediscrete}} becomes:
In the limiting case when $\Delta s \to 0$, Eq. \ref{eq:cosinediscrete} becomes:
\begin{equation}
%\frac{d \mathcal{L}_f(\vp, t)}{d t} = -\left< \vu(\vp), \vu(\vp + s(t)\vu(\vp)) \right>
\frac{d \mathcal{L}_f(\vp, s)}{d s} = -\left< \vu(\vl_\vp(0)), \vu(\vl_\vp(s)) \right>
\label{eq:odecos}
\end{equation}
%Since $s(t)$ is linearly related to $t$ from our formulation, using a change of variables, we get:
%\begin{equation}
%\frac{d \mathcal{L}_f(\vp, s)}{d s} = -\left< \vu(\vp), \vu(\vp + s\vu(\vp)) \right>
%\label{eq:odecos}
%\end{equation}
where $\mathcal{L}_f(\vp, 0) = 0$ and $\vl_\vp(0) = \vp$. Our final alignment loss $\mathcal{L}_f(\vp)$ is defined as an  integral of the Eq. \ref{eq:odecos} and Eq. \ref{eq:deltal},
%which is solved as:  % $\mathcal{L}_f() = \mathcal{L}_f(\vp, 2r(\vp))$ which is the solution of Equation \ref{eq:odecos}.
\begin{equation}
    \begin{bmatrix}
    \mathcal{L}_f(\vp) \\
    \vl_\vp \\
    \end{bmatrix}
    = 
    \begin{bmatrix}
    0 \\ \vp 
    \end{bmatrix} + 
    \int_0^{2r(\vp)} \begin{bmatrix}
    -\left< \vu(\vl_\vp(0)), \vu(\vl_\vp(s)) \right> \\
    \vu(\vp) \\
    \end{bmatrix} ds
    \label{eq:bigodecos}
\end{equation}
where $\mathcal{L}_f(\vp)$ is shorthand notation for $\mathcal{L}_f(\vp, 2r(\vp))$ and $\vl_\vp$ is short for $\vl_\vp(2r(\vp))$.
Eq. \ref{eq:bigodecos} is solved using a differentiable ODE solver.
%Note that the second argument to $\mathcal{L}_f$ is equal to $2r(\vp)$ (instead of being a constant) to ensure that larger line segments are considered for larger tube-like structures and similarly for smaller line segments.
Note that, we used $2r(\vp)$ as an upper limit in  integral so that the length of the traversal path is proportional to the size of the vessel.  
%Next, we describe a loss function to detect the presence of bifurcation angles, and use the existing template alignment idea to predict the bifurcation flow fields. 
%%% Bifurcations
\subsection{Bifurcation}
Bifurcation point (BP) is a point on a vessel where the main vessel splits into two sub-vessels.
Similar to vessel flow $\vu$, we predict bifurcation flow fields $\vb_1$ and $\vb_2$ as vector fields representing the two directions of the bifurcation. Although the BP doesn't match the canonical template T, the incoming vessel and the two sub-vessels should match T. We maximize the profile symmetry between these three segments, by minimizing the following bifurcation loss,

\begin{equation}
    \mathcal{L}_b(\vp) = 1 - \frac{\sum_{\vv(\vp) \in \{ \vu(\vp), \vb_1(\vp), \vb_2(\vp) \}} S(I, T \circ \Phi_{\{r(\vp), \vv(\vp)\}}(\vp)) }{3}
    \label{eq:bifurc}
\end{equation}

Note that, in the absence of bifurcation, $\vb_1(\vp) = \vb_2(\vp) = -\vu(\vp)$ minimizes the loss function.
Hence in practice, we can replace the loss function in Eq. \ref{eq:alignment} with Eq. \ref{eq:bifurc}. Also, we parameterized the neural network such that the bifurcation flow fields $\vb_1$ and $\vb_2$ will always satisfy $\left< \vb_1(\vp), \vu(\vp) \right> \le 0$ and $\left< \vb_2(\vp), \vu(\vp) \right> \le 0$ for all $\vp \in \Omega$. This constraint prevents the bifurcation directions and vessel flow from collapsing into a single direction.

\subsection{Intensity and vesselness consistency losses}
Template matching approach to find vessel points may result in false positives due to background noise or artifacts. To make our model robust towards such local intensity abnormalities, we propose a regularization loss that encourages uniform intensity along the vessel. 
%Similar to before, we take $T$ positive, equally spaced step sizes $s_1 \le s_2 \ldots \le s_T$ for which we want to measure the intensity error.
%If the intensity error after considering $t$ step sizes is $\mathcal{L}_i(\vp, t)$, the alignment loss after considering $t+1$ step sizes is:
%$$ 
%\mathcal{L}_i(\vp, t+1) = \mathcal{L}_i(\vp, t) + \left[ I(\vp) - I(\vp + s_{t+1}\vu(\vp)) \right]^2
%$$
Similar to the formulation for path continuity in Eq.~\ref{eq:cosinediscrete}, we define an intensity alignment loss along our traversal path as,
\begin{equation}
\mathcal{L}_i(\vp, s + \Delta s) = \mathcal{L}_i(\vp, s) + \| I(\vl_\vp(s)) - I(\vl_\vp(s + \Delta s)) \|_2 
\label{eq:discreteli}
\end{equation}
Since $\Delta s$ is small and $\vl_\vp(s + \Delta s) = \vl_\vp(s) + \Delta s\cdot \vu(\vp)$, the right hand side of the equation can be written as
$$
I(\vl_\vp(s + \Delta s)) = I(\vl_\vp(s)) + \nabla I(\vl_\vp(s))^T \vu(\vp) \Delta s 
$$
where $\nabla I$ is the gradient of the image. 
Subsituting this equation and taking the limit $\Delta s \to 0$ in Eq. \ref{eq:discreteli}, we get:
\begin{equation}
    \frac{d \mathcal{L}_i(\vp, s)}{ds} = \Big \| \nabla I(\vl_\vp(s))^T \vu(\vp) \Big\|_2
    \label{eq:odei}
\end{equation}
Similarly, we used the vesselness metric $V(\vp)$ to minimize the  vesselness alignment error $\mathcal{L}_v(\vp, s)$ given by:
\begin{equation}
\frac{d \mathcal{L}_v(\vp, s)}{ds} = \Big \| \nabla V(\vl_\vp(s))^T \vu(\vp) \Big\|_2
\label{eq:odev}
\end{equation}
 We simultaneously solve Eq. \ref{eq:odei} and Eq. \ref{eq:odev} as:
\begin{equation}
   \begin{bmatrix}
   \mathcal{L}_i(\vp) \\
   \mathcal{L}_v(\vp) \\
   \vl_\vp \\
   \end{bmatrix} 
   = \begin{bmatrix}
   0 \\ 0 \\ \vp 
   \end{bmatrix} + 
   \bigints_0^{2r(\vp)} \begin{bmatrix}
   \Big \| \nabla I(\vl_\vp(s))^T \vu(\vp) \Big \| \\ 
   \Big \| \nabla V(\vl_\vp(s))^T \vu(\vp) \Big \| \\
   \vu(\vp)
   \end{bmatrix} ds
\end{equation}
where $\mathcal{L}_i(\vp)$ and $\mathcal{L}_v(\vp)$ are shorthand notations for $\mathcal{L}_i(\vp, 2r(\vp))$ and $\mathcal{L}_v(\vp, 2r(\vp))$ respectively.
The integrals can be computed using a differentiable ODE solver.
The reasoning for choice of upper limit in the integral is the same as that of the path continuity loss.

%Similar to Equation \ref{eq:cosinediscrete}, we take this equation to the limiting case and after a change of variables like before, we get:
%\begin{equation}
    %\frac{d \mathcal{L}_i(\vp, s)}{ds} = \left[ I(\vp) - I(\vp  + s\vu(\vp)) \right]^2
%\end{equation}
%We can solve this ODE with the initial value $\mathcal{L}_i(\vp, 0) = 0, \mathcal{L}_v(\vp, 0) = 0, \vl_\vp(0) = \vp$ to get the intensity error along the vessel flow segment which is equal to $\mathcal{L}_i(\vp, 2r(\vp))$. \\
%We can use a similar idea to take the error of the vesselness function along the vessel flow segment as well.
%This is due to the assumption that the tube-like structures are continuous and therefore do not change their contrast drastically along the tube.
%If this error is measured by $\mathcal{L}_v(\vp, s)$, it satisfies the ODE:
%\begin{equation}
    %\frac{d \mathcal{L}_v(\vp, s)}{ds} = \left[ V(\vp) - V(\vp  + s\vu(\vp)) \right]^2
%\end{equation}
%We compute the total vesselness error along the vessel flow segment which is given by $\mathcal{L}_v(\vp, 2r(\vp))$.



\subsection{Robust vesselness metric}
The primary caveat of commonly used vesselness functions is that they also have a high response to other structures that are geometrically very different from tubular structures.
One such example is a ridge, which is usually indicative of a flat surface.
Although a ridge is very different from a vessel, commonly used vesselness functions \cite{unsup} \cite{unsup} \cite{unsup} 

\subsection{Postprocessing}

%aq* We are going to define some of the properties of the tube-like structures such as vessels to come up with a self-supervised algorithm.

%* (1) The first property is vessel continuity. The idea is that vessel can be viewed as continious path. We use a vector field which we call \emph{vessels flow}.

%* (2) The second property build on top of the first property. The flow characterize the directionality of the tube. Orthogonal profile with respect to the flow is radially symmetric around the axis defined by the flow.

%* (3) The third property the bifurcation possibility. For example, vessel have tree-like structure that include bifurcations. We also use the first property to model the bifurcation. We view bifurcation as splitting flow. The bifurcation is also modeled as a vector field which deviates from the vessel flow whereever we have bifurcation. 

%* Our formulation also has a few regularization enforcing other consistencies of the tube-like structure. For example, the intensity of the vessels should not change drastically if we walk along the vessel flow. 

%* The idea is shown in \figurename{\ref{fig:framework}}


%* We start the method section with explainign the second property followed by vessel-flow and formulation of the birfurcation. 

%\textbf{Notation:} 
%We are going to use $I: \Omega \rightarrow \mathbb{R}$ to denote input image where $\Omega \subset \sR^d$ is the input domain and $d$ is the dimensionality of the image. We $\vu : \Omega \rightarrow \sS^{d-1}$ to denote the tube-flow where $\sS^{d-1}$ denotes unit hypersphere of embedded in $d$-dimensional space. For the bifurcation, we define two more flows $\vb_1: \Omega \rightarrow \sS^{d-1}$ and $\vb_2 : \Omega \rightarrow \sS^{d-1}$ each representing the directionality of the birfurcation. Furthermore, we define a scalar field $r: \Omega \rightarrow \sR^{+}$ defining the radius of the tube. We use $T: \Omega \rightarrow \sR$ to denote protypical template for the tube-like structure. We use $\Phi_{\theta}: \Omega \rightarrow \Omega $ is a transformation parametrized by $\theta$.

%\subsection{Second Property}
%* To determine the radious of the tube, we locally match the profile of the tube with a canonical template. 

%* At the given point $p \in \Omega$, We apply an affine transformation $\Phi_{\theta}$ parameterized by $\theta$ on the template $T$ where the parameters are \emph{locally} specified by we do that by the vessel-flow $\vu$ and scale it locally with scalar radius $r$. 
%\begin{equation}
    %I(p) \approx T \circ \Phi_{(r(p),\vu(p) )} (p)
%\end{equation}


%\subsection{First Property}
%
%\subsection{Third Property}
%
%\subsection{Regularization}
%
%\subsection{Post Processing}


==> sections/related_work_v1.tex <==

% \section{Related Work}
  
  Automatic vessel segmentation is a challenging problem, given that the vascular networks are complex multi-level tree structures with high variability in local geometry, curvature and radius, that further varies across modalities and subjects. 
  %The complexity is further increased by varying contrast and the present of pathologies, noise, or artifacts. 
 % Hence, manual segmentation is a tedious, time-consuming process, which is subject to inter-observer variability. 
Consequently, research has focused on developing specially designed vessel segmentation pipelines for a particular modality including 2D retinography~\cite{fraz2012blood} and 3D thoracic CT~\cite{rudyanto2014comparing}. 
%and MRA~\cite{lesage2009review}.
Many state-of-the-art unsupervised vessel segmentation methods, uses classical Hessian-based scale-space filters~\cite{frangi,hessian,sato} along with other  processing techniques  such as particle sampling~\cite{estepar2012computational} and region growing~\cite{yu2008multiscale} to achieve their best results. In contrast, we propose an end-to-end vessel segmentation model that generalizes across modalities and dimensions.  %,oksuz2013region,yu2008multiscale} and model-based methods~\cite{krissian2000model}. But these methods often have limited robustness, and extensive pre and post-processing steps are required for better results~\cite{mendonca2006segmentation, yang2012automatic,Martinez1999,truc2009vessel}
%In this paper, we present an 


%Some prominent unsupervised strategies for vessel segmentation includes, Hessian-based multi-scale analysis~\cite{frangi,hessian,sato}, 
%multi-scale analysis~\cite{vlachos2010multi}, 
%region-growing methods~\cite{QIANZHAO20142437,AlDiri2009,5193288} and centerline detection
 
Our work is inspired from matched filter response (MFR) method~\cite{chaudhuri1989detection} which assumes vessel to be piece-wise linear segments and used multiple Gaussian kernels to identify vessel-like structures. 
As the Gaussian assumption may fail and the filters have high sensitivity towards noise, different variants of MFR~\cite{stare}%,oliveira2016unsupervised,sreejini2015improved,kumar2016retinal} 
and several post-processing techniques~\cite{memari2019retinal}
%jiang2003adaptive, memari2019retinal,vermeer2004model} 
have been proposed to improve MFR.
Our paper is an attempt to generalize the MF concept by using  convolutional neural network (CNN) to define each vessel point in-terms of radius and direction of flow, rather than any explicit assumption. 
We further consider path continuity constraints to extract the local geometry of the tube, and intensity regularization to maintain robustness to noise and other artifacts. 

Recently, various deep learning (DL) based techniques have been proposed for vessel segmentation~\cite{SoomroReview2019}. Though DL based supervised methods have achieved high performance, due to scarcity of annotated data, researchers are now exploring un-supervised and self-supervised methods~\cite{taleb20203d,zhou2019models}.
